Unsupervised Learning of Global Factors in Deep Generative Models

We present a novel deep generative model based on non i.i.d. variational autoencoders that captures global dependencies among observations in a fully unsupervised fashion. In contrast to the recent semi-supervised alternatives for global modeling in deep generative models, our approach combines a mixture model in the local or data-dependent space and a global Gaussian latent variable, which lead us to obtain three particular insights. First, the induced latent global space captures interpretable disentangled representations with no user-defined regularization in the evidence lower bound (as in $\beta$-VAE and its generalizations). Second, we show that the model performs domain alignment to find correlations and interpolate between different databases. Finally, we study the ability of the global space to discriminate between groups of observations with non-trivial underlying structures, such as face images with shared attributes or defined sequences of digits images.

==> background.tex <==
\subsection{Background: Variational Autoencoders}

\begin{figure}[htbp]
	\centering
	\subfigure[VAE]{\includegraphics[width=0.17\linewidth]{figs/vae}}
	\qquad \qquad \qquad
	\subfigure[GMVAE]{\includegraphics[width=0.4\linewidth]{figs/gmvae}}
	\caption{Generative (solid line) and inference (dashed lines) of VAE and GMVAE. } 
	\label{fig:vae_gmvae}
\end{figure}

%We denote some input data as $\textbf{X} = \{\textbf{x}_1, ..., \textbf{x}_N \} \subseteq \mathbb{R}^D$ and the corresponding latent codes as $\textbf{Z}= \{ \textbf{z}_1, ... \textbf{z}_N\} \subseteq \mathbb{R}^d $. 
The Variational Autoencoder (VAE, \cite{kingma2013auto}) is a deep generative model with a latent variable $\textbf{z}$ that generates data $\textbf{x}$ and joint distribution $p_\theta(\textbf{x}, \textbf{z})$, where we define $p_\theta(\textbf{z})$ as a prior and $p_\theta(\textbf{x} \vert \textbf{z})$ as a likelihood. The likelihood is \textit{decoded} using a neural network that outputs the distribution parameters given an input code. The posterior $p(\textbf{z} \vert \textbf{x})$ is approximated by a recognition model $q_\phi(\textbf{z} \vert \textbf{x})$ parametrized by an \textit{encoder} network (\cite{rezende2014stochastic}).  Thanks to the use of encoder and decoder networks, VAEs make use of amortized inference to approximate the true posterior. Furthermore, using the reparametrization trick, the Evidence Lower Bound (ELBO) on the log likelihood is trained stochastically by using Stochastic Variational Inference, and thus, data is injected to the model in minibatches.

More recently, in order to mitigate the problem of overgeneralization in multimodal data, the Gaussian Mixture VAE (GMVAE, \cite{dilokthanakul2016deep}) has been proposed to perform clustering in latent space using a Gaussian Mixture. The ELBO function for GMVAE adds two new regularizers w.r.t. to the Vanilla VAE:
\begin{equation}
\begin{gathered}
\mathcal{L} (\theta, \phi; \textbf{x}, \textbf{z}, \boldsymbol{\beta}, \textbf{d}) = \mathbb{E}_{q(\textbf{z} \vert \textbf{x})} \left[ \log(p(\textbf{x} \vert \textbf{z})) \right] 
- KL\left( q(\textbf{z} \vert \textbf{x}) \Vert p(\textbf{z}) \right) \\
- KL\left( q(\boldsymbol{\beta} \vert \textbf{x}) \Vert p(\boldsymbol{\beta}) \right)
- KL\left( q(\textbf{d} \vert \boldsymbol{\beta}, \textbf{z}) \Vert p(\boldsymbol{\textbf{d}}) \right)
\end{gathered}
\end{equation}
  The prior for $\boldsymbol{\beta}$ is typically chosen as isotropic Gaussian and the prior for the discrete $\textbf{d}$ as uniform, with probability $1/K$, where $K$ is the number of components. As showed in Figure \ref{fig:vae_gmvae}, $\boldsymbol{\beta}$ acts a code that is projected into one component beteween $K$. The reconstruction term and the first regularizer work exactly the same way than in VAE. The second divergence acts as a regularizer for the noise $\boldsymbol{\beta}$, and the third regularizer is for the discrete variable $\textbf{d}$.


\begin{figure}[htbp]
	\centering
	\subfigure[Generative model]{\includegraphics[height=0.32\linewidth]{figs/gen}}
	\qquad \qquad \qquad
	\subfigure[Inference model]{\includegraphics[height=0.32\linewidth]{figs/inf}}
	\caption{Generative (left) and inference (right) models of GGMVAE. } 
	\label{fig:ggmvae}
\end{figure}

